Error Interference in Quantum Simulation

Understanding algorithmic error accumulation in quantum simulation is crucial due to its fundamental significance and practical applications in simulating quantum many-body system dynamics. Conventional theories typically apply the triangle inequality to provide an upper bound for the error. However, these often yield overly conservative and inaccurate estimates as they neglect error interference -- a phenomenon where errors in different segments can destructively interfere. Here, we introduce a novel method that directly estimates the long-time algorithmic errors with multiple segments, thereby establishing a comprehensive framework for characterizing algorithmic error interference. We identify the sufficient and necessary condition for strict error interference and introduce the concept of approximate error interference, which is more broadly applicable to scenarios such as power-law interaction models, the Fermi-Hubbard model, and higher-order Trotter formulas. Our work demonstrates significant improvements over prior ones and opens new avenues for error analysis in quantum simulation, offering potential advancements in both theoretical algorithm design and experimental implementation of Hamiltonian simulation.

==> macros.tex <==
% Draft?
\def\draft{0}  % 1 for draft version (eg including author notes and structure symbols), 0 for non-draft version

% AMS packages
\usepackage{amsmath,amsfonts,amsthm,amssymb,bm,bbm}
\usepackage{pdfpages}

% TikZ
\usepackage{tikz}
\usetikzlibrary{math}
\usetikzlibrary{shapes.geometric}

% Page margins
\usepackage[margin = 0.8in]{geometry}

% Quantum circuit
% preventing conflicts with \gate in fig-circuit.tex, we use savesym
%\usepackage{savesym}
%\usepackage{qcircuit}
%rename \gate of qcircuit to \origgate
%\savesymbol{gate}

% Hypertext
\usepackage[colorlinks = true]{hyperref}
% Title and authors
%\hypersetup{
%  pdftitle = {}
%  pdfauthor = {}
%}
% Color definitions
\definecolor{darkred}  {rgb}{0.5,0,0}
\definecolor{darkblue} {rgb}{0,0,0.5}
\definecolor{darkgreen}{rgb}{0,0.5,0}
% Color links
\hypersetup{
  urlcolor   = blue,         % color of external links
  linkcolor  = darkblue,     % color of internal links
  citecolor  = darkgreen,    % color of links to bibliography
  filecolor  = darkred       % color of file links
}

% Clever references
\usepackage{cleveref}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{proposition}{Proposition}{Propositions}
\crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{section}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{table}{Table}{Tables}
\crefname{example}{Example}{Examples}

%% Theorem environments
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{example}[theorem]{Example}
%\newtheorem*{observation}{Observation}
%\newtheorem*{theorem*}{Theorem}
%% separately number
\newtheorem{theorem}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem*{observation}{Observation}
\newtheorem*{theorem*}{Theorem}

% Operators
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\cc}{cc}

% Sets
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\U}[1]{\mathrm{U}(#1)}

% Tensors
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}

% Expectation
\newcommand{\E}{\mathbb{E}}

% Matrices
\newcommand{\mx}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\smx}[1]{\bigl(\begin{smallmatrix}#1\end{smallmatrix}\bigr)}

% Paired delimiters
\usepackage{mathtools}
\mathtoolsset{centercolon}
%\DeclarePairedDelimiter{\set}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\of}{\lparen}{\rparen}
\DeclarePairedDelimiter{\sof}{\lbrack}{\rbrack}

% Short-cuts
\newcommand{\ct}{^{\dagger}}
\newcommand{\tp}{^{\mathsf{T}}}
\newcommand{\x}{\otimes}
\newcommand{\xp}[1]{^{\otimes #1}}

% Notation
\newcommand{\Part}{\mathcal{P}}
\newcommand{\EPR}{\mathrm{EPR}}
\newcommand{\dd}{\vec{d}}
\renewcommand{\th}[1]{#1^\text{th}}

% H gate
\newsavebox{\Hgate}
\savebox{\Hgate}{$H:=\smx{1&1\\1&-1}/\sqrt{2}$}
% S gate
\newsavebox{\Sgate}
\savebox{\Sgate}{$S:=\smx{1&0\\0&i}$}

% Notes
\ifnum\draft=1
\newcommand{\anote}[1]{\textcolor{magenta}{(\textbf{Aram:} #1)}}
\newcommand{\mnote}[1]{\textcolor{magenta}{(\textbf{Maris:} #1)}}
\newcommand{\tnote}[1]{\textcolor{magenta}{(\textbf{Tianyi:} #1)}}
\newcommand{\xnote}[1]{\textcolor{magenta}{(\textbf{Xiaodi:} #1)}}
\else
\newcommand{\anote}[1]{}
\newcommand{\mnote}[1]{}
\newcommand{\tnote}[1]{}
\newcommand{\xnote}[1]{}
\fi

%Structure Symoble
\ifnum \draft=1
\newcommand{\Lone}[1]{{\color{red} \textbf{#1}}}
\newcommand{\Ltwo}[1]{{\color{blue} #1}}
\else
\newcommand{\Lone}[1]{#1}
\newcommand{\Ltwo}[1]{}
\fi

\newcommand{\sect}[1]{\vspace{1mm}\noindent \textbf{#1.}}
\usepackage[numbers, square]{natbib}
\usepackage{multirow}
\parskip = 0.02in

\newlength{\blank}
\settowidth{\blank}{\emph{~}}
\renewenvironment{proof}[1][{\hspace{-\blank}}]{{\noindent\textbf{Proof~{#1}.\ }}}{\hfill\qed}
%\newenvironment{proof}[1][Proof]{\noindent\textbf{Proof~#1.} }{\hfill\qed}
%\newcommand{\ket}[1]{|#1\rangle}
%\newcommand{\bra}[1]{\langle#1|}
%\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\ketbra}[2]{| #1 \rangle\langle #2 |}
\newcommand{\proj}[1]{| #1 \rangle\langle #1 |}
%\input{tcilatex}

% % Align := properly in math mode
% \mathchardef\ordinarycolon\mathcode`\:
% \mathcode`\:=\string"8000
% \def\vcentcolon{\mathrel{\mathop\ordinarycolon}}
% \begingroup \catcode`\:=\active
%   \lowercase{\endgroup
%   \let :\vcentcolon
%   }

\newcommand{\nc}{\newcommand}
\nc{\rnc}{\renewcommand}
\nc{\beq}{\begin{equation}}
\nc{\eeq}{{\end{equation}}}
\nc{\beqa}{\begin{eqnarray}}
\nc{\eeqa}{\end{eqnarray}}
\nc{\lbar}[1]{\overline{#1}}
%\nc{\bra}[1]{\langle#1|}
%\nc{\ket}[1]{|#1\rangle}
%\nc{\ketbra}[2]{|#1\rangle\!\langle#2|}
%\nc{\braket}[2]{\langle#1|#2\rangle}
%\nc{\proj}[1]{| #1\rangle\!\langle #1 |}
\nc{\avg}[1]{\langle#1\rangle}
%\rnc{\max}{\operatorname{max}}
\nc{\Rank}{\operatorname{Rank}}
\nc{\smfrac}[2]{\mbox{$\frac{#1}{#2}$}}
%\nc{\tr}{\operatorname{Tr}}
% \newcommand{\Tr}{\operatorname{Tr}}
\nc{\ox}{\otimes}
%\nc{\dag}{\dagger}
\nc{\dn}{\downarrow}
\nc{\cA}{\mathcal{A}}
\nc{\cB}{\mathcal{B}}
\nc{\cC}{\mathcal{C}}
\nc{\cD}{\mathcal{D}}
\nc{\cE}{\mathcal{E}}
\nc{\cF}{\mathcal{F}}
\nc{\cG}{\mathcal{G}}
\nc{\cH}{\mathcal{H}}
\nc{\cI}{\mathcal{I}}
\nc{\cJ}{\mathcal{J}}
\nc{\cK}{\mathcal{K}}
\nc{\cL}{\mathcal{L}}
\nc{\cM}{\mathcal{M}}
\nc{\cN}{\mathcal{N}}
\nc{\cO}{\mathcal{O}}
\nc{\cP}{\mathcal{P}}
\nc{\cR}{\mathcal{R}}
\nc{\cS}{\mathcal{S}}
\nc{\cT}{\mathcal{T}}
\nc{\cX}{\mathcal{X}}
\nc{\cZ}{\mathcal{Z}}
\nc{\csupp}{{\operatorname{csupp}}}
\nc{\qsupp}{{\operatorname{qsupp}}}
\nc{\var}{\operatorname{var}}
\nc{\rar}{\rightarrow}
\nc{\lrar}{\longrightarrow}
\nc{\polylog}{\operatorname{polylog}}
%\nc{\1}{{\openone}}
\nc{\1}{\mathbbm{1}}
%\nc{\id}{{\operatorname{id}}}
\nc{\RR}{{{\mathbb R}}}
\nc{\CC}{{{\mathbb C}}}
\nc{\FF}{{{\mathbb F}}}
\nc{\NN}{{{\mathbb N}}}
\nc{\ZZ}{{{\mathbb Z}}}
\nc{\PP}{{{\mathbb P}}}
\nc{\QQ}{{{\mathbb Q}}}
\nc{\UU}{{{\mathbb U}}}
\nc{\EE}{{{\mathbb E}}}

\nc{\GOCC}{{\mathrm{GOCC}}}
\nc{\Wplus}{{\mathrm{W+}}}

%\nc{\qed}{{$\hfill\Box$}}
\newcommand{\ip}[2]{\langle #1|#2\rangle}
%outer product
\newcommand{\op}[2]{|#1\rangle \langle #2|}

%\newcommand{\1}{{\openone}}
\newcommand{\slocc}{\overset{\underset{\mathrm{SLOCC}}{}}{\longrightarrow}}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\mc}{\mathcal}
\newcommand{\Rm}{\mathbb{R}^m}
\newcommand{\Rn}{\mathbb{R}^n}
% \newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\pdiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddiv}[2]{\frac{d #1}{d #2}}
%\newcommand{\tr}{\text{Tr}}
\newcommand{\mf}[1]{\mathfrak{ #1}}
\newcommand{\Ex}{\text{Exp}}

\newcommand{\edit}[1]{{\color{red} #1}}

\renewenvironment{proof}{\medskip\noindent\textbf{Proof.}}{\hfill$\blacksquare$\medskip}
%AW: New environment for "Proof of Theorem X" etc
\newenvironment{proof-of}[1]{\medskip\noindent\textbf{Proof of {#1}.}}{\hfill$\blacksquare$\medskip}


